CASA-NLU: Context-Aware Self-Attentive Natural Language Understanding for Task-Oriented Chatbots

Natural Language Understanding (NLU) is a core component of dialog systems. It typically involves two tasks - intent classification (IC) and slot labeling (SL), which are then followed by a dialogue management (DM) component. Such NLU systems cater to utterances in isolation, thus pushing the problem of context management to DM. However, contextual information is critical to the correct prediction of intents and slots in a conversation. Prior work on contextual NLU has been limited in terms of the types of contextual signals used and the understanding of their impact on the model. In this work, we propose a context-aware self-attentive NLU (CASA-NLU) model that uses multiple signals, such as previous intents, slots, dialog acts and utterances over a variable context window, in addition to the current user utterance. CASA-NLU outperforms a recurrent contextual NLU baseline on two conversational datasets, yielding a gain of up to 7% on the IC task for one of the datasets. Moreover, a non-contextual variant of CASA-NLU achieves state-of-the-art performance for IC task on standard public datasets - Snips and ATIS.

==> dataset_f.tex <==
\subsection{Datasets}
\label{sec:dataset_f}

% NOT USED . SEE EXPERIMENTS
Since there are no existing public datasets for contextual \pretty{Ic} and \pretty{Sl} task, we use two in-house datasets for evaluation - \textbf{booking} dataset,\footnote{We plan to release this dataset} which is a variation on \pretty{Dstc}-2 dataset \cite{williams2014dialog}, and \textbf{cable} dataset, a synthetically created multi-goal conversational dataset. 
 %Table \ref{data_table} shows statistics of these four datasets.
The \emph{Booking} dataset contains 9351 training utterances and 6727 test utterances, with 19 intents and 5 slot types. \emph{Cable} dataset comprises 1856 training utterances, 1814 validation utterances and 1836 test utterances, with 21 intents and 26 slot types.\footnote{Detailed Data statistics provided in supplementary material}
In addition, we also evaluate the model on non-contextual \pretty{Ic-Sl} public datasets - \pretty{Atis} \cite{hemphill90} and \pretty{Snips} \cite{coucke2018snips}.



==> model_f.tex <==

%%% NOT USED ANYMORE. SEE CDISAN_F %%%


\section{CASA NLU: Context-Aware Self-Attentive NLU}
\label{sec:model_f}

% Below is the formalization of contextual NLU framework. For a conversation with n turns, we have: \\
% %Agent Utterances: $A = \{a_1, a_2, \ldots, a_n\}$\\
% User Utterances: $U = \{u_1, u_2, \ldots, u_n\}$  \\
% Intents: $I = \{i_1, i_2, \ldots, i_n\}$ \\
% Slot Labels: $SL = \{sl_1, sl_2, \ldots, sl_n\}$  \\
% Dialog Acts\footnote{Dialog Act signifies the actions taken by agent like Close (when an intent is fulfilled) ConfirmIntent, ElicitSlot etc. }: $DA = \{da_1, da_2, \ldots, da_n\}$ 
% %Slot Elicitation\footnote{Slot Elicitation signifies the slots to elicit when the dialog act is ElicitSlot}: $SLE = \{sle_1, sle_2, \ldots, sle_n\}$ \\

% For a traditional non-contextual NLU system, for turn $t$, the intent and slots are given by:
% $$i_t, sl_t = f_{no\_context}(u_t)$$
% where, $f_{no\_context}$ is typically an encoder-decoder architecture with attention \cite{joint_ic_sl, Goo2018SlotGatedMF}.

% For the contextual NLU system with a context window, i.e. length of contextual history, of $K$, for turn $t$, the intent and slots are given by:
% $$i_t, sl_t = f_{context}(u_t, c_t)$$
% where, 
% \begin{equation}
% \begin{split}
% c_t = & < u_{t-K}, \ldots, u_{t-1}, da_{t-K+1}, \ldots, da_t,\\
% %& da_{t-K+1}, \ldots, da_t,\\
% & i_{t-K}, \ldots, i_{t-1} >
% \end{split}
% \end{equation}

% \begin{equation}
% \begin{split}
% c_t = & < a_{t-K+1}, \ldots, a_t, u_{t-K}, \ldots, u_{t-1},\\
% & da_{t-K+1}, \ldots, da_t, i_{t-K}, \ldots, i_{t-1},\\
% & sle_{t-K}, \ldots, sle_{t} >
% \end{split}
% \end{equation}

Our architecture is divided into three sub sections - signal encoding, context fusion and IC-SL predictions
%To learn this $f_{context}$, we propose two different models that take turn history over $K$ turns  into account along with the current utterance: contextual self-attention model (cSA) and contextual Memory network (cMemN)

% To solve the task of contextual NLU, we propose two different models that take turn history over long period into account along with the current utterance: contextual self-attention model (cSA) and memory network (MemN).
% Dialog history includes utterances from user and agent sides in each turn. For $n$ turns, we denote agent prompts as $A = \{a_1, a_2, \ldots, a_n\}$, while user utterances as $U = \{u_1, u_2, \ldots, u_n\}$. 
\input{cdisan_f}
%\input{memnw}








